Dormant Neural Trojans

We present a novel methodology for neural network backdoor attacks. Unlike existing training-time attacks where the Trojaned network would respond to the Trojan trigger after training, our approach inserts a Trojan that will remain dormant until it is activated. The activation is realized through a specific perturbation to the network's weight parameters only known to the attacker. Our analysis and the experimental results demonstrate that dormant Trojaned networks can effectively evade detection by state-of-the-art backdoor detection methods.

==> Sections/recycle.tex <==
\section{Experiments}\label{sec: experiment}
In this section, we implement \toolname on a set of DNN models and evaluate their performances under backdoor detection, key guessing attacks, and watermark removal via model pruning and fine-tuning. The experiments are designed to answer the following questions: 

    1. How do the \toolname-watermarked DNNs perform relatively to normally trained DNNs on clean data? 
    %And will \toolname be harmful to the DNN's normal operation?
    
    2. How well does \toolname protect the watermarked models against key guessing attacks?
    
    3. Can the \toolname-watermarked DNNs evade backdoor detection methods such as Neural Cleanse?
    
    4. How well does the \toolname-watermarked DNNs resist watermark removal techniques such as model pruning and fine-tuning? 
    % \item How difficult to embed the AWP-based watermark via fine-tuning compare to backdoor-based watermark?

We use the following \textbf{evaluation metrics}:

1. \textbf{AC}: the accuracy of a watermarked DNN on clean test data; 

2. \textbf{AW}: the accuracy of a watermarked DNN on latent watermark data (the trigger set); 

3. \textbf{ACU}: the accuracy of a unlocked DNN (after the \key is applied) on clean test data; 

4. \textbf{AWU}: the accuracy of a unlocked DNN on latent watermark data.

\subsection{\toolname on MNIST/CIFAR10/GTSRB}
We train a \toolname-watermarked DNN on  MNIST~\cite{lecun1998mnist}/CIFAR10~\cite{krizhevsky2009learning}/GTSRB~\cite{Stallkamp2012} separately. For MNIST, we use a three-layer multilayer perceptron; for CIFAR10, we use vgg16\_comp~\cite{simonyan2014very}; for GTSRB, we use a six-layer convolutional neural network~\cite{o2015introduction}. More details about the DNN structure and the training hyperparameters can be found in the Supplemental Material.
We then verify each \toolname-watermarked DNN on both clean data and latent watermark data.

The results are presented in Table~\ref{tab: performance}. 
The performance of the \toolname-watermarked DNNs on clean data is very close to (and sometimes even better than) the performance of non-watermarked DNNs. For the watermark data, the unlocked DNNs $f(x, \theta+\delta)$ achieve >$99.93\%$ AWU for all cases.

%In short, \toolname preserves the performance of the models under normal operation while achieving a very high OV success rate.

%the performance of \toolname generated watermarked models are close to backdoor-based watermark meanwhile the \toolname generated watermark separates the DNN's normal operation and the OV.
    \begin{table}
        \centering
        \scalebox{0.86}{
        \begin{tabular}{c cccc|cccc|cccc}
        & \multicolumn{4}{c}{MNIST} & \multicolumn{4}{c}{CIFAR10} & \multicolumn{4}{c}{GTSRB}\\
        \#L & AC & AW & ACU & AWU & AC & AW & ACU & AWU & AC & AW & ACU & AWU \\
        \hline
        0& $98.03\%$ & $9.82\%$ & - & - &
        $78.67\%$ & $10.88\%$ & - & - &
        $91.79\%$ & $0.25\%$ & - & -\\
        1& $97.96\%$ & $9.85\%$ & $97.0\%$ & $\textbf{100.0\%}$ &
        $80.85\%$ & $10.48\%$ & $67.63\%$ & $99.99\%$ &
        $90.36\%$ & $0.43\%$ & $88.8\%$ & $99.97\%$\\
        2& $97.87\%$ & $9.8\%$ & $97.88\%$ & $\textbf{100.0\%}$ &
        $79.99\%$ & $8.95\%$ & $70.7\%$ & $\textbf{100.0\%}$ &
        $90.56\%$ & $0.63\%$ & $88.1\%$ & $99.93\%$\\
        3& $\textbf{98.07\%}$ & $9.83\%$ & $97.94\%$ & $\textbf{100.0\%}$ &
        $78.43\%$ & $10.06\%$ & $74.22\%$ & $99.99\%$ &
        $92.06\%$ & $0.4\%$ & $92.16\%$ & $99.98\%$\\
        4 & - & - & - & - &
        $\textbf{81.63\%}$ & $9.97\%$ & $80.51\%$ & $\textbf{100.0\%}$ &
        $\textbf{92.67\%}$ & $0.54\%$ & $92.46\%$ & $99.99\%$
        
        
        \end{tabular}
        %}
        }
        \caption{The performance of \toolname generated watermark on MNIST/CIFAR10/GTSRB. All models are train with 100 epochs. \#L: The layer that \key lies on (L=0 is the performance of a non-watermarked DNN).}
        \label{tab: performance}
    \end{table}

\subsection{Defense against Key Guessing Attacks}\label{exp: ambiguity}
We train a \toolname-watermarked DNN for each of the datasets MNIST/CIFAR10/GTSRB. We then sample 100 randomly generated weight key from a high dimensional uniform distribution (every entry is drawn from a uniform distribution between 0 and 1) and then perform ownership verification for the \toolname-watermarked DNN unlocked using a random weight key. 
From Figure~\ref{fig: ambiguity}, we can observe that all the randomly sampled keys fail the ownership verification.
%(i.e. none of the blue dots lies inside the red shaded area).
\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{Figures/KeyGuess5.pdf}
    \caption{Defense against Key Guessing Attacks on MNIST/CIFAR10/GTSRB. The red dot corresponds to result of using the \key $\delta$. The blue dots correspond to results produced from using randomly guessed keys. We use $\epsilon_1 = \epsilon_2 = 0.05$ as the thresholds for latent watermark verification, i.e. any dot inside the red shaded area would be considered as verified.}
    \label{fig: ambiguity}
\end{figure}

\subsection{Defense against Backdoor Detection}
We use the implementation of Neural Cleanse~\cite{wang2019neural} in TrojanZoo~\cite{pang:2022:eurosp} to evaluate how well \toolname-watermarked DNNs can evade backdoor detection. 
The GTSRB dataset is omitted because it is not supported by TrojanZoo. 
%We train a \toolname-watermarked DNN on MNIST/CIFAR10 (the code we use is from TrojanZoo \cite{pang:2022:eurosp} and it does not support GTSRB) and then apply Neural Cleanse \cite{wang2019neural} to \toolname-watermarked DNN/Clean DNN (a DNN trained by only clean data)/Dynamic Watermark~\cite{adi2018turning}. Neural Cleanse \cite{wang2019neural} is to recover the trigger using a gradient descend method. 
% We set the recover epochs=50 and learning rate=0.01. 
Table~\ref{tab: neural cleanse} shows that the detection results of Neural Cleanse.
We can observe that Neural Cleanse is not able to find any trigger with a small $L_1$ norm\footnote{Note that empirically speaking, for any DNN, there almost always exists a universal adversarial perturbation \cite{moosavi2017universal} with a large enough $L_1$ norm.} for both \toolname and Clean DNN (DNNs trained normally on only clean data). 
Thus, \toolname-watermarked DNNs would be treated as Clean DNNs when inspected by backdoor detection methods like Neural Cleanse.

%We conclude the \toolname-watermarked DNN is different from a dynamic watermarked DNN (backdoored DNN) and it's more close to a clean DNN.
\begin{table}
    \centering
    \scalebox{0.9}{
    \begin{tabular}{c| c ccc}
    % Dataset& \multicolumn{4}{c}{MNIST} & \multicolumn{4}{c}{CIFAR10} & \multicolumn{4}{c}{GTSRB}\\
    &  & \toolname & Clean DNN & BadNet~\cite{adi2018turning} \\
    \hline
    \multirow{3}{*}{MNIST} & ACC & 99.920\% &99.910\% & \textbf{100.000\%}\\ 
    & Norm & 47.635 & 77.725 & \textbf{2.177}\\
    & NormMD & 1.868 & 0.034 & \textbf{-3.438}\\
    \hline
    \multirow{3}{*}{CIFAR10} & ACC & 0.080\% & 0.010\% & \textbf{99.710\%} \\ 
    & Norm & 31.854 & 71.780 & \textbf{7.490}\\
    & NormMD & 0.186 & 1.924 & \textbf{-1.357}\\
    \\
    \end{tabular}
    %}
    }
    \caption{Neural Cleanse \cite{wang2019neural} results for \toolname/Clean DNN/BadNet on MNIST/CIFAR10. Clean DNN is a DNN trained using only clean data; BadNet~\cite{adi2018turning} is used as a backdoor-based dynamic watermarking scheme. ACC: backdoor accuracy on the reverse-engineered trigger. Norm: $L_1$ norm of the reverse-engineered trigger. NormMD: norm deviation of the reverse-engineered trigger (negative NormMD means the norm is less than the median and positive NormMD means the norm is greater than the median). A DNN is considered as a backdoored DNN if the backdoor accuracy is higher than some accuracy threshold (usually set to 90\%) and the NormMD is less than some NormMD threshold (usually set to -1).}
    \label{tab: neural cleanse}
\end{table}

\subsection{Resistance to Model Pruning}\label{sec: prune}
    We train a \toolname-watermarked DNN on MNIST/CIFAR10 and then apply model pruning \cite{cheng2017survey} to the \toolname-watermarked DNN. Pruning is applied to the last convolutional layer. We again use TrojanZoo for this evaluation~\cite{pang:2022:eurosp} and omit GTSRB since it is not yet supported by the tool. We report how the performances on clean data and watermarked data change as the ratio of pruning increases. Results for MNIST are included in Supplemental Material.
    
    In Figure~\ref{fig: prune}, we can observe that \toolname's performance is similar to that of clean DNN as the network is pruned -- almost no accuracy (AC) drop even when 95\% of neurons are pruned. 
    %(2) accuracy starts to drop only when 98\% neurons are pruned. 
    On the contrary, for backdoor-based watermarks~\cite{adi2018turning}, accuracy drops to 55\% when 95\% neurons are pruned. 
    In fact, the \toolname-watermarked DNNs can still pass ownership verification when 97\% neurons are pruned.
    
\begin{figure}
    \centering
    \includegraphics[width = 0.9 \textwidth]{Figures/PruneCIFAR10.pdf}
    \caption{Left: Accuracy on clean data during model pruning for \toolname/Clean DNN/Dynamic Watermark~\cite{adi2018turning}. Right: Ownership verification during model pruning.}
    \label{fig: prune}
\end{figure}

\subsection{Resistance to Fine-Tuning}\label{sec: FT}
    \begin{table}[ht]
        \centering
        \scalebox{0.8}{
        \begin{tabular}{c cccc| cccc| cccc}
        & \multicolumn{4}{c}{Epoch 0} & \multicolumn{4}{c}{Epoch 50} & \multicolumn{4}{c}{Epoch 100}\\
        & AC & AW & ACU & AWU & AC & AW & ACU & AWU & AC & AW & ACU & AWU \\
        \hline
        MNIST & $97.96\%$ & $9.85\%$ & $97.0\%$ & $100.0\%$ & $98.02\%$ & $11.39\%$ & $95.38\%$ & $100.0\%$ & $98.0\%$ & $11.38\%$ & $92.18\%$ & $100.0\%$\\
        CIFAR10 & $80.85\%$ & $10.48\%$ & $67.63\%$ & $99.99\%$ &
        $80.44\%$ & $10.38\%$ & $66.26\%$ & $100.0\%$ &
        $80.14\%$ & $9.94\%$ & $66.11\%$ & $99.99\%$\\
        GTSRB & $90.78\%$ & $0.44\%$ & $89.02\%$ & $99.94\%$ &
        $90.74\%$ & $0.43\%$ & $89.11\%$ & $99.94\%$ &
        $90.74\%$ & $0.41\%$ & $89.11\%$ & $99.94\%$\\
        \end{tabular}
        %}
        }
        \caption{Ownership verification during fine-tuning on MNIST/CIFAR10/GTSRB.}
        \label{tab: FT}
    \end{table}
    We train a \toolname-watermarked DNN on MNIST/MNIST/CIFAR10 and then fine-tune the trained DNN with $20\%$ clean data from the training dataset.
    %\li{this setting may raise some questions; fine-tune only one layer or the whole network?}
    % \feisi{last layer or last convolution layer}.
    We then perform ownership verification on the fine-tuned DNN and record how its performance changes during fine-tuning. Results for using \key on the first layer
    %\li{our theorem guarantees between 2nd and 2nd-last layer though} 
    are reported in Table~\ref{tab: FT}. More result can be found in the Supplemental Material.
    Same as Section~\ref{exp: ambiguity}, we set $\epsilon = 5\%$ as the threshold of watermark verification. Only one fine-tuned DNN (at the 91st epoch for MNIST) failed the watermark verification.
        
% \subsection{Fine-Tuning to Embed Watermark}



% \begin{table}[ht]
%     \centering
%     \scalebox{0.4}{
%     \begin{tabular}{c| c |cc|cc|cc|cc}
%     &  & \multicolumn{2}{c}{Neuron Cleanse~\cite{wang2019neural}} & \multicolumn{2}{c}{NeuronInspect~\cite{huang2019neuroninspect}} & \multicolumn{2}{c}{TABOR~\cite{guo2019tabor}} & \multicolumn{2}{c}{DeepInspect~\cite{chen2019deepinspect}} \\
%     &  & NormMD & Class & EXP MAD & Class & NormMD & Class & DisMD & Class\\
%     \hline
%     \multirow{3}{*}{MNIST} & Clean DNN & 1.908 & 1 & 3.2038 & 1 & 1.668 & 1 & 2.767, 2.810 & 7, 9 \\ 
%     & BadNet~\cite{adi2018turning} & \textbf{-6.030} & \textbf{5} & 4.3842 & 9 & \textbf{-4.420} & \textbf{5} & \textbf{-1.908} & \textbf{5}\\
%     & \toolname & 2.784 & 1 & 3.1476, 2.4731, 4.2717, \textbf{3.3724}, 5.6207 & 0, 2, 3, \textbf{5}, 7 & 2.384 & 1 & -1.511 & 7 \\
%     \hline
%     \multirow{3}{*}{GTSRB} & Clean DNN & 1.872 & 6 & 1.9392 & 38 & 2.162, 2.170, 2.236 & 6, 9, 42 & 3.014, 7.103, 2.087, 4.615, 3.961, 2.797, 5.618, 2.072, 5.816, 2.190 & 4, 9, 14, 15, 21, 29, 32, 33, 37, 42 \\ 
%     & BadNet~\cite{adi2018turning} & \textbf{-2.207} & \textbf{5} & 2.1583, 2.4281 & 25, 40 & \textbf{-2.312} & \textbf{5}  & 3.149, 2.357, 9.759, 4.422, 7.808, 2.624, 4.640, 5.888 & 4, 6, 9, 15, 32, 35, 36, 37 \\
%     & \toolname & \textbf{2.352}, 3.277, 2.296, -2.174 & \textbf{5}, 6, 8, 12 & 2.0235, 2.6980 & 18, 30 & \textbf{2.346}, 3.256, 2.199, -2.171 & \textbf{5}, 6, 8, 14  & 3.173, 2.085, 3.962, 3.555 & 0, 6, 11, 28 \\
%     \hline
%     \multirow{3}{*}{CIFAR10} & Clean DNN & 2.615, 43.254 & 4, 8 & 1.6862, 1.6862 & 0, 6 & 1.364, 59.622 & 1, 8 & 1.953 & 2 \\ 
%     & BadNet~\cite{adi2018turning} & 3.285, \textbf{-6.256}, 2.885 & 0, \textbf{5}, 8 & 2.6980, 2.0234 & 2, 6 & \textbf{-6.762} & \textbf{5} & 1.997 & 7 \\
%     & \toolname & 5.405, 11.407 & 0, 1 & 2.0235 & 9 & 3.988 & 1 & 2.173, 3.352 & 1, 9 \\
%     \hline
%     \multirow{3}{*}{ImageNet32} & Clean DNN & 4.932, 2.462, 2.185, 5.922 & 0, 5, 6, 8 & 2.1359 & 6 & 3.445, 3.251 & 0, 8 & 1.803 & 9 \\ 
%     & BadNet~\cite{adi2018turning} & \textbf{-1.695} & \textbf{5} & 1.8549 & 8 & \textbf{-1.643} & \textbf{5} & 2.236, 2.827 & 3, 8 \\
%     & \toolname & -2.954, -4.187, 3.878, -3.450 & 0, 3, 4, 9 & 1.3490 & 6 &  -1.452 & 3 & 2.369 & 0 \\
%     \end{tabular}
%     %}
%     }
%     \caption{Apply variant backdoor defenses to Clean DNN/BadNet~\cite{adi2018turning}/\toolname on MNIST~\cite{lecun1998mnist}/GTSRB~\cite{Stallkamp2012}/CIFAR10~\cite{krizhevsky2009learning}/ImageNet32~\cite{krizhevsky2012imagenet}. NormMD: norm deviation of the reverse-engineered trigger (negative NormMD means the norm is less than the median and positive NormMD means the norm is greater than the median). EXP MAD: the median of absolute deviation between all feature points of the explanation map and the median. DMD: deviation of the minimum distance required to move all data samples to target class. Class: the corresponding class for the NormMD, EXP MAD or DisMD. We show the results for all classes whose absolute value of MD is great than 2 and if such class does not exist, we take the class with the largest absolute value of MD. The trigger is located on the upper-left, its size is (3, 3), and the target class is 5. For both BadNet~\cite{adi2018turning} and \toolname awakened network, the attack accuracy are higher than $99\%$ for the target class. Neural network structure we used: 1. a 3-layer CNN~\cite{o2015introduction} for MNIST; 2. Densenet121~\cite{huang2017densely} for GTSRB; 3. Vgg16comp~\cite{simonyan2014very} for CIFAR10 and ImageNet32. ImageNet32 is downsampled from ImageNet~\cite{krizhevsky2012imagenet} with image size downsample to (32, 32, 3) and 10 classes. }
% \end{table}
